The carbon-rich type Ic supernova 2016adj in the iconic dust lane of Centaurus A: signatures of interaction with circumstellar hydrogen?

We present a comprehensive data set of supernova (SN) 2016adj located within the central dust lane of Centaurus A. SN 2016adj is significantly reddened and after correcting the peak apparent $B$-band magnitude ($m_B = 17.48\pm0.05$) for Milky Way reddening and our inferred host-galaxy reddening parameters (i.e., $R_{V}^{host} = 5.7\pm0.7$ and $A_{V}^{host} = 6.3\pm0.2$), we estimate it reached a peak absolute magnitude of $M_B \sim -18$. Detailed inspection of the optical/NIR spectroscopic time-series reveals a carbon-rich SN Ic and not a SN Ib/IIb as previously suggested in the literature. The NIR spectra shows prevalent carbon-monoxide formation occurring already by +41 days past $B$-band maximum, which is $\approx 11$ days earlier than previously reported in the literature for this object. Interestingly around two months past maximum, the NIR spectrum of SN~2016adj begins to exhibit H features, with a +97~d medium resolution spectrum revealing both Paschen and Bracket lines with absorption minima of $\sim 2000$ km/s, full-width-half-maximum emission velocities of $\sim 1000$ km/s, and emission line ratios consistent with a dense emission region. We speculate these attributes are due to circumstellar interaction (CSI) between the rapidly expanding SN ejecta and a H-rich shell of material formed during the pre-SN phase. A bolometric light curve is constructed and a semi-analytical model fit suggests the supernova synthesized 0.5 solar masses of $^{56}$Ni and ejected 4.2 solar masses of material, though these values should be approached with caution given the large uncertainties associated with the adopted reddening parameters, possible CSI contamination, and known light echo emission. Finally, inspection of Hubble Space Telescope archival data yielded no progenitor detection.

==> co.tex <==



\bigskip



{\bf PAH remarks on the Mass of CO above the photosphere:}

For the following, I assume T=3900 K, v=2050m/sec, with
error bars of $\pm 100K$ and $200 km/sec$, respectively.
The $\delta$-Ceph. distance has been used to be $D=3.42 \pm 0.18 Mpc=\approx 1.03 10^{25} cm $.
No reddening correction has been applied which, thus,
may result in a linear shift of the mass of $M_{CO}$.

 No detailed simulations have been performed for the LCs and spectra, and the CO  
profiles within an overtone are insensitive to $\rho $. It would take observations of the  
fundamental band to break this degeneracy. Here, the basic goal is to estimate $\rho $ an 
 to obtain $M_{CO}$.

We assume a power law profile for the C/O core, i.e. $\rho \propto r^{-n}$.
typically $n=2...5$ are found in the CO-rich layers of massive stars 
SN1993 \citep{2003MNRAS.345..111C,1998ApJ...502..737C,1993A&A...275L..29H}.
(Remark: Same is true for any model from Woosley ... Heger because the cores are
close to polytropes.)


To estimate the lower limit of the CO mass, $M_{CO}$, we assumed
flux being produced in an isothermal layer. It is a lower limit because
we see only the optically thin layer or, better, the layers outside
"CO-photosphere". $M_{CO}$ is the mass outside this photosphere
\citep{2021ApJ...908..232R}.

 $M_{CO}$ is based on the peak CO astrophysical flux as observed 
$F_{obs}\approx 1.7~10^{-15}$ erg~s$^{-1} cm^{-2} \AA^{-1}$ at distance $D$ compared to the 
emitted flux by an unknown mass $M_{CO}$ in the object. 

 In principle, detailed radiation transport is required \citep{1995ApJ...444..831H,2000AJ....119.2968G} but, 
to obtain an estimate, it is not necessary. Instead, we integrate the CO emissivity over the volume.   
For our parameters, we find the black body 
$BB(23000\AA, 3900 K)=4.66~10^{12}  erg~s^{-1} cm^{-2} \AA^{-1}$.


First step is to determine $R_{CO}=r(\tau_{CO}=1)$ at 97 days after maximum light, i.e.
$$R_{CO}=v_{CO} (t+t_{max}) \approx 1.7~10^{15} cm$$.
with $R_{CO}$ is the radius at optical depth 1 in the peak of the first overtone of  CO.

Next step is to determine the density $\rho_{CO}$ iteratively assuming $\kappa(R_{CO})$  
with $\kappa (CO)=2. particles/g$ as starting value. Note that $\kappa $ changes by a factor of about 3 with 
the range $\Delta T= \pm 100K$.
 For temperatures considered here and instead using but guided by the explicit tables, 
we use $\kappa(CO) \propto 1/\rho$  for efficiency, and obtain
$\rho_{CO} \approx (n-1)/R_{CO}*kappa_(R_{CO})$. For the lowest n, $M_{CO} \approx 2.5 \times 10^{-4} M_\odot$.
Depending on the density slope and radiative transport effects,  $M_{CO}$ may be larger by a factor of 1 to 2 
whether the CO-emission originates in a large volume or close to the photosphere, respectively.
 Moreover, due to uncertainties in distance (quadratic), density slope ($\propto n(max)/n(min)$), and the uncertainties in
the radius $R_{CO}$ due to $v(CO)$ (10\%?) and detailed abundance structure, this value is uncertain by  
an additional factor of $\approx 2 ... 3$. Note that, in future, we will use
RTE and additional constraints to estimate $M_{CO}$. Here, it  should be regarded as an order of magnitude only. 

{\bf PAH end of remarks on the Mass of CO above the photosphere}
\bigskip

